Report on the AAPM Grand Challenge on deep generative modeling for learning medical image statistics

The findings of the 2023 AAPM Grand Challenge on Deep Generative Modeling for Learning Medical Image Statistics are reported in this Special Report. The goal of this challenge was to promote the development of deep generative models (DGMs) for medical imaging and to emphasize the need for their domain-relevant assessment via the analysis of relevant image statistics. As part of this Grand Challenge, a training dataset was developed based on 3D anthropomorphic breast phantoms from the VICTRE virtual imaging toolbox. A two-stage evaluation procedure consisting of a preliminary check for memorization and image quality (based on the Frechet Inception distance (FID)), and a second stage evaluating the reproducibility of image statistics corresponding to domain-relevant radiomic features was developed. A summary measure was employed to rank the submissions. Additional analyses of submissions was performed to assess DGM performance specific to individual feature families, and to identify various artifacts. 58 submissions from 12 unique users were received for this Challenge. The top-ranked submission employed a conditional latent diffusion model, whereas the joint runners-up employed a generative adversarial network, followed by another network for image superresolution. We observed that the overall ranking of the top 9 submissions according to our evaluation method (i) did not match the FID-based ranking, and (ii) differed with respect to individual feature families. Another important finding from our additional analyses was that different DGMs demonstrated similar kinds of artifacts. This Grand Challenge highlighted the need for domain-specific evaluation to further DGM design as well as deployment. It also demonstrated that the specification of a DGM may differ depending on its intended use.

==> do_not_use.tex <==
% \textit{Pradeep} (group 1064), \textit{mukundkhanna123} (1067), 

% \underline{\textit{Pradeep} (Group 1064) and \textit{mukundkhanna123} (Group 1067):} % (1064-Pradeep.pdf)

% \textit{Pradeep} trained a class-conditional StyleGAN-XL [SG-XL link here] on the provided data. The input labels were generated by segregating the data into four classes using \textit{k}-nearest neighbor (KNN) clustering based on the provided public metric features, and those extracted from breast density classifiers pre-trained on screening mammography exams [Breast Density Classifier link here]. A progressive training strategy was employed to train the GAN until the FID score converged. At inference, the generated images were downscaled and then super-resolved using an existing superresolution method to improve the clarity of the ligaments [RealESRGAN link here]. Additionally, \textit{mukundkhanna123} also employed a threshold-based memorization rejection strategy.  A total time of $~120$ minutes on an NVIDIA A40 GPU was reported for generating the required 10,000 images.

% % \textit{Pradeep} used StyleGAN-XL [SG-XL link here] as the data generative model. The model was trained on the entire dataset with additional data labels. The data labels were generated by segregating the training dataset into 4 different clusters using \textit{k} nearest neighbor (KNN) with Euclidean distance as metric based on three sets of features: the handcrafted features provided in the public metrics, image features and histogram-based features extracted from two pre-trained breast density classifiers trained on screening mammography exams [Breast Density Classifier link here]. To speed up the convergence, a progressive training schedule was used starting from a image size of $16\times16$ and doubled each time till reaching $512\times512$. In each of the steps the StyleGAN-XL model was optimized for $1,000$ iterations till FID stops improving. During inference, seeds of $0-2499$ were used for 1st class, $2500-4999$ for 2nd class and so on to generate $2,500$ images for each class. In addition, the ligament tissue was further improved by using a super resolution network RealESRGAN [RealESRGAN link here]. This was done by resizing StyleGAN-XL generated $512\times512$ images to $256\times256$ and then upscaling them to $512\times512$ again using the super resolution network. Regarding computation cost, the group reported that StyleGAN-xl took about $100$ minutes to generate $10,000$ images on A40 and RealESRGAN took about $20$ minutes to upscale $10,000$ images on A40.


% \hspace{-8mm}\underline{\textit{lisun} (Group 1065):} %(1065-lisun.pdf)

% \textit{lisun} trained a StyleGAN2 with adaptive discriminator augmentation (ADA) strategies such as pixel blitting [ref], rotation and translation, more general geometric transformations, and color transforms. The group did not report the computational cost at inference. % Regarding computation cost, the group reported that the model was trained for $1.5$ days from scratch using 2 NVIDIA A6000 GPUs.

% % \textit{lisun} used StyleGAN2 as the data generative model. They leveraged StyleGAN2 with adaptive discriminator augmentation. During the training, the batch size was set to $64$, the learning rate was set to $0.0015$ for both generator and discriminator and the number of iterations was $75,000$. Augmentation strategies including pixel blitting (x-flip, $90^{\text{o}}$ rotation, translation), more general geometric transformations, color transforms. Regarding computation cost, the group reported that the model was trained for $1.5$ days from scratch using 2 NVIDIA A6000 GPUs.

% \hspace{-8mm}\underline{\textit{weidec} (Group 1066):} %(1066-weidec.pdf)

% \textit{weidec} employed a latent diffusion model [medfusion link] which embeds an image into a latent space using a variational autoencoder (VAE), and then trains a conditional UNet-based diffusion model in the latent space. A combination of $\ell_1$, SSIM, perceptual loss, and KL divergence was used to train the VAE. The UNet diffusion model was trained to minimize an $\ell_2$ loss function with classifier-free guidance with the total breast area and log fat-to-glandular tissue ratio ($\log(F/G)$) as conditioning inputs. During interference, conditioning inputs were drawn from the training data and a deep diffusion implicit modeling (DDIM) scheme was used to generate image samples with reduced timesteps. Finally,  postprocessing steps such as thresholding and filtering were applied to remove image sampling artifacts. The group reported a total time of 10 hours to generate 10,000 images using one NVIDIA V100 16GB GPU.

% % \textit{weidec} used a latent diffusion model [medfusion link] as the data generative model. The latent diffusion model featured two networks: a variational autoencoder (VAE) which embeds each image into a latent space, and a UNet diffusion model that is trained to map samples from a standard Gaussian to this latent space. The VAE was a convolutional autoencoder with an encoder composed of a convolutional block and two downsampling blocks that embeded each $512\times512$ images into a $128\times128\times8$ latent space. It was trained for 30 epochs to minimize a loss combining L1, SSIM, perceptual loss and a KL divergence between latent distribution and a standard Gaussian. The UNet diffusion model was trained for $75$ epochs to minimize an L2 loss function with classifier-free guidance to condition each training sample with its total breast area and log fat-to-glandular tissue ratio ($\log(F/G)$). During interference, a deep diffusion implicit modeling scheme was used to generate image samples with fewer ($150$) timesteps and variance fixed. Conditional labels [area, $\log(F/G)$] were drawn from the training dataset to generate samples of similar size and glandular density as the training dataset and fed to the denoising model. These samples were denoised in the latent space with the diffusion model and then converted to the image space with the decoder. Finally, some classical image postprocessing steps, such as thresholding and filtering, were applied to remove image sampling artifacts. Regarding computation cost, the group estimated that it took about 10 hours for this model to generate 10,000 images using one NVIDIA V100 16GB GPU.

% % \hspace{-8mm}\underline{\textit{mukunskhanna123} (Group 1067):} %(1067-mukundkhanna123.pdf)

% % \textit{mukunskhanna123} used almost the same method and implementation as Pradeep did. The only difference is that a memorization rejection was implemented during the StyleGAN-XL training process: A threshold of $0.13$ was used and any generated images that were sufficiently close to the training dataset were not passed to the generator loss function. 

% \hspace{-8mm}\underline{\textit{xiaoerlaigeid} (Group 1033)} % Sub id:1033 (xiaoerlaigeid)

% \textit{xiaoerlaigeid} employed a two-staged approach. In the first stage, a denoising diffusion GAN (DDG) was used to generate low-resolution images. Subsequently, a super-resolution technique was employed to up-sample the DDG output [ESR-GAN ref]. The two-staged approach reduced the computational and memory costs of training and inference. The models were trained using a 24 GB Nvidia GeForce RTX 3090 GPU. However, this group did not report or estimate their computation time.

% % \textit{xiaoerlaigeid} employed a two-staged approach to train on the challenge dataset. In the first stage, Denoising Diffusion GAN (DDG) was used to generate low-resolution images. Subsequently, a super-resolution technique was employed in the second step to up-sample the DDG output. In particular, DDG was used to generate $128 \times 256$ breast images. These outputs were then passed into the ESR-GAN model to, ultimately, get an output image sized $512 \times 512$. This two-staged approach was primarily employed to overcome the issues related to a diffusion model’s cost for training, inference time, and memory-based hardware limitation. The diffusion and super-resolution models were trained using an Nvidia GeForce RTX 3090 GPU with 24 GB of memory models. However, this group did not report or estimate their computation time.

% \hspace{-8mm}\underline{\textit{nkamath} (Group 1048):} %Sub id: 1048 (nkamath)

% \textit{nkamath} trained three state-of-the-art generative models (StyleGAN2, StyleGAN3, SWAGAN) in parallel using the challenge dataset. They proceeded with a heuristics approach to re-tune some important parameters corresponding to each model to get a low FID and KS-statistics score simultaneously. Accordingly, it was determined that StyleGAN2 model obtained the best performance (with an FID score of $22.56$ and KS statistics score of $0.0134$).

% Regarding the StyleGAN2-based training, the PyTorch implementation of StyleGAN2 was used [SG2 link here]. \textit{nkamath} deemed that the training dataset was sufficient and did not train using the StyleGAN2-ada version. Also, it was found that the generated images were plagued with artifacts when the default augmentations were enabled. Likewise, three different R1 $\gamma$ values (i.e., $2$, $10$, and $100$) were experimented and it was found that setting the R1 $\gamma$ as 2 yielded the lowest FID score. The model training was performed on four V100 16GB GPUs with batch size $96$ for $9.072$ million images. Additional training parameters were set in accordance with the base configuration of `paper256’ [link here].

% Regarding the StyleGAN3-based training, the best FID and KS statistics scores \textit{nkamath} obtained were $118.27$ and $0.319$, respectively. This includes gamma experimentation with $0.5$, $1$, $2$, $4$, $8$, $10$, and $100$. Based on their observations, \textit{nkamath} concluded that StyleGAN3 is a newer version of StyleGAN that tries to tackle the texture sticking issue that occurs during the morphing transition (e.g., morphing from one face to another face) in StyleGAN2. More concretely, StyleGAN3 tries to make the transition animation more natural (i.e., smooths out some features) by redesigning the network layers and introducing positional references (i.e., adding distortions). However, this may not be appropriate for all the four breast types provided in the challenge dataset (that exhibit high fidelity and sharpness).
% Finally, regarding SWAGAN-based training, \textit{nkamath} obtained the best performance with an FID score of $27$ and a KS statistics score of $0.067$. \textit{nkamath} obtained this performance by setting the default hyperparameter setting as provided in the repository at [link here]. The training was performed using 4 GPUs for 24 hours (corresponding to the checkpoint $210,000$). 

% \hspace{-8mm} \underline{\textit{mckellwoodland} (Group 1060):} %Sub id 1060 (mckellwoodland)

% \textit{mckellwoodland} employed the StyleGAN2 network to train on the DGM challenge dataset using NVlab’s GitHub repository [SG3 link]. To overcome the data size limitation, \textit{mckellwoodland} experimented with transfer learning from pre-trained weights (from the Flickr-Faces-HQ Dataset (FFHQ) provided at [weights link here] and adaptive discriminator augmentation (ADA).

% Regarding the hyperparameter setting, mixed precision was disabled and was set to $0.9$ in the Adam optimizer. A hyperparameter search was performed over the regularization parameter $\gamma$. The rest of the parameters were left in their original default settings. Finally, each experimental setup was trained for three independent runs/initializations to obtain the model that yielded images with the smallest FID score.

% Contrary to their initial judgment/strategy to train StyleGAN2 with transfer learning, the lowest FID score of $1.58$ was actually achieved in an experimental setup without transfer learning. This experimental setup consisted of ADA with no transfer learning and default regularization parameter ($\gamma=8.2$) for 10 million images. However, it was found that this experimental setup was volatile. The same setup gave FID scores of 13.8 and 3.36 in the second and third runs/initializations, respectively. Moreover, it was observed that the model trained from the second run generated images with inverted colors. Nonetheless, \textit{mckellwoodland} proceeded with the same best-performing experimental setup (i.e., ADA, no transfer learning, and default regularization parameter $\gamma$) for 100 million images, with an early stopping of 10 million images, and for five random initializations. Of these five independent runs, the network with the lowest FID (1.34) was saved as their final model. This strategy allowed a further decrease of the FID score by $0.24$. Regarding computation cost, the group reported that it took less than 10 minutes on a V100 GPU to generate $10,000$ images.

% \hspace{-8mm} \underline{\textit{jpvteixeira} (Group 1061):} %sub id 1061 (jpvteixeira)

% \textit{jpvteixeira} used a latent diffusion model called Medfusion to train on the challenge dataset. Medfusion model is based on the Stable Diffusion model, consisting of a variational autoencoder and a denoising diffusion probabilistic model. No pre-trained weights were used to train their generative model. Perceptual loss was calculated using the VGG weights for the LPIPS perceiver (used in their autoencoder part). Finally, samples were generated with a denoising diffusion implicit model with $t=300$ steps. The code is available at [link here] and weights at [link here]. Regarding computation time, the group reported that it took approximately eight hours and thirty minutes to generate 10,000 images.

% \hspace{-8mm} \underline{\textit{yshi20} (Group 1062):} %Sub id:1062 (yshi20)

% \textit{yshi20} used the StyleGAN2-ada (i.e., the adaptive discriminator augmentation model incorporated in the StyleGAN2 backbone) to train on the challenge data. Some of the important training parameter settings include R1 $\gamma$ as $6.6$, batch size of $8$, learning rate as $0.0025$, and augmentation strength as $0.6$. Augmentations such as pixel blitting, image filtering, geometric transformation, and color transformation was incorporated. FID score was used to monitor the robustness of the StyleGAN2-ada as the training iteration progressed. Subsequently, it was deemed that the model achieved its best performance at $7.4$ million images seen in training. The training was completed using a single GPU. Finally, some post-processing operations were employed on the images generated from the trained StyleGAN2-ada model. These included replacing pixels with intensity values lower than forty by zero. To remove artifacts at the corner of the generated images, image intensity along the borders of these images\textemdash specifically corresponding to 5 pixels in width from the edge of the image\textemdash was replaced with zero values. This group did not report or estimate their computation time.

% \begin{table}[htb]\label{tab:classwise}
% \caption{Class-based analyses of submissions}
% \vspace{5pt}
% \begin{tabular}{@{}lllll@{}}
% \toprule
% User & Rank                 & Class prevalence (\%)                         & Class coverage            & Class density \\
% \textit{wiedec}             & \textbf{1} & 10.26, 40.78, 38.95, 10.01       & 0.86, 0.97, 0.96, 0.97    & 1.02, 1.00, 1.00, 1.02 \\
% \textit{Pradeep}            & \textbf{2} & 10.46, 39.54, 40.37, 9.63        & 0.00, 0.85, 0.94, 0.77    & 0.96, 0.99, 0.99, 0.99 \\
% \textit{mukundkhanna123}    & \textbf{3} & 10.36, 39.68, 40.31, 9.65        & 0.00, 0.80, 0.91, 0.74    & 0.00, 0.98, 0.99, 0.96 \\
% \textit{xiaoerlaigeid}      & \textbf{4} & 3.04, 29.85, 55.07, 12.04        & 0.00, 0.25, 0.41, 0.15    & 0.00, 0.72, 0.62, 0.22 \\
% \textit{lisun}              & \textbf{5} & 9.01, 38.91, 35.18, 16.90        & 0.00, 0.27, 0.34, 0.25    & 0.00, 0.35,  0.49, 0.24 \\
% \textit{jpvteixeira}        & \textbf{6} & 10.57, 47.76, 38.23, 3.44        & 0.00, 0.12, 0.19, 0.11    & 0.00, 0.19, 0.28, 0.32 \\
% \textit{mckellwoodland}     & \textbf{7} & 10.77, 39.99, 40.31, 8.93        & 0.00, 0.25, 0.66, 0.62    & 0.00, 0.66, 0.83, 0.69 \\
% \textit{yshi20}             & \textbf{8} & 11.09, 43.10, 35.28, 10.53       & 0.00, 0.27, 0.38, 0.31    & 0.00, 0.38, 0.47, 0.17 \\
% \textit{nkamath}            & \textbf{9} & 14.47, 41.85, 39.97, 3.71        & 0.00, 0.63, 0.60, 0.43,   & 0.00, 0.74, 0.55, 0.55 \\

% \bottomrule
% \end{tabular}
% \vspace{10pt}
% \end{table}

% User & Rank                 & Class prevalence (\%)                         & Class coverage            & Class density \\
% \textit{wiedec}             & \textbf{1} & 10, 41, 39, 10       & 0.9, 1, 1, 1    & 1, 1, 1, 1 \\
% \textit{Pradeep}            & \textbf{2} & 10, 40, 40, 10        & 0, 0.8, 0.9, 0.8    & 1, 1, 1, 1 \\
% \textit{mukundkhanna123}    & \textbf{3} & 10, 40, 40, 10        & 0, 0.8, 0.9, 0.7    & 0, 1, 1, 1 \\
% \textit{xiaoerlaigeid}      & \textbf{4} & 3, 30, 55, 12        & 0, 0.2, 0.4, 0.1    & 0, 0.7, 0.6, 0.2 \\
% \textit{lisun}              & \textbf{5} & 9, 39, 35, 17        & 0, 0.3, 0.3, 0.2    & 0, 0.3,  0.5, 0.2 \\
% % \textit{jpvteixeira}        & \textbf{6} & 11, 48, 38, 3        & 0, 0.1, 0.2, 0.1    & 0, 0.2, 0.3, 0.3 \\
% \textit{mckellwoodland}     & \textbf{7} & 11, 40, 40, 9        & 0, 0.2, 0.7, 0.6    & 0, 0.7, 0.8, 0.7 \\
% \textit{yshi20}             & \textbf{8} & 11, 43, 35, 11       & 0, 0.3, 0.4, 0.3    & 0, 0.4, 0.5, 0.2 \\
% \textit{nkamath}            & \textbf{9} & 14, 42, 40, 4        & 0, 0.6, 0.6, 0.4,   & 0, 0.7, 0.5, 0.5 \\

% Rate of flipped images in ensemble: 30 to 50 \% for two submissions.
% Rate of boundary breaks: 0.5 to 1\% in 3 submissions
% Rate of background texture: 0 in 2 submissions, 4\% in 2 submissions, 75\% in 1 submission, 100\% in 3 submissions

==> timeline.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]\label{tab:timeline}
\caption{Timeline for the DGM-Image challenge}
\vspace{5pt}
\begin{tabular}{@{}ll@{}}
\toprule
January 13, 2023 & Challenge announced, participant registration opened                         \\
January 16, 2023 & Training set released                                                        \\
May 19, 2023     & Deadline for Phase 1 submission                                              \\
May 29, 2023     & Deadline for Phase 2 submission                                              \\
June 14, 2023    & Participants and top-ranked finishers contacted with results                 \\
July 27, 2023    & Top two finishers presented their results at the AAPM annual meeting \\ \bottomrule
\end{tabular}
\vspace{10pt}
\end{table}


